Monodromy results for abelian surfaces and K3 surfaces with bad reduction

The purpose of this paper is to prove a local p-adic monodromy theorem for ordinary abelian surfaces and K3 surfaces with bad reduction in characteristic p. As an application, we get a finiteness result for the reduction of their Hecke orbits in the case of type II supersingular reduction.

==> extratext.tex <==
%\begin{prop}\label{raynaudk3}
%Let $X$ be a $K3$ surface over $\mathbb{C}$ with bad reduction and $KS(X)$ be the associated Kuga Satake abelian variety. Let $T\rightarrow G_{KS}\rightarrow A_{KS}$ be the Raynaud extension of $KS(X)$. Then the abelian part of the Raynaud extension $A_{KS}$
% is isomorphic to a product of $d/2$ copies of an elliptic curve $E$ over $\mathbb{C}$
 
% \end{prop}
 
%\begin{proof}
    
%We  follow \cite{ksabvar} for the following construction. \textcolor{purple}{nevermind this proves that the special fibre splits not the generic fibre.}
%Let $V$ be the fibre over a point in the disc $\Delta^{*}$. Suppose $N\in \mathfrak{so}\simeq \wedge^2V$ is the monodromy operator on $V$ satisfying $N^3=0.$ For the case that we're interested in, is when $N^2 = 0$ that corresponds to the Kuga-Satake abelian variety having semi-abelian reduction. The associated weight filtration is

%$$0\subset W_{1}V\subset W_2V\subset W_3V\subset V$$
%Since $W_{1}V$ is $2$-dimensional, we note that the weight one Hodge structure coming from this filtration corresponds to an elliptic curve.
%Let $H = \mathcal{C}l(V)$ be its corresponding clifford algebra with dimension $d =2^r$ where $r$ is the dimension of $V$. We let $N^{\prime} = \eta(N)$ be its corresponding monodromy operator given by the image of $N$ under the map:
%$\eta: \mathfrak{so}(V,q)\rightarrow \mathcal{C}l(V,q)$.
%The associated weight filtration
%$$0\subset W_0H\subset W_1 H\subset H$$
%where $W_0H = ker N^{\prime}$ and $W_1H = im N^{\prime}$. We know that the dimension of $W_1H = 3d/4$ and that of $W_0H = d/4.$ We have the following decomposition of $H$ 

%$$\mathcal{C}l(V) = \mathcal{C}l (U\oplus U^{\prime},q|_{U\oplus U^{\prime}})\otimes \mathcal{C}l(V^{\prime},q|_{V^{\prime}})$$
%Here $U = \langle{e_2,e_3}\rangle$ such that $q(e_2,e_2) = q(e_3,e_3) = 2$ and $q(e_2, e_3) = 0.$ Similarly, $U_3 = \langle{e_1,e_4}\rangle$ such that $q(e_1,e_1) = q(e_4,e_4) = 2$ and $q(e_1, e_4) = 0.$
%Hence, $\mathcal{C}l(V) = \mathcal{C}l (U\oplus U^{\prime},q|_{U\oplus U^{\prime}})$ is $16$ dimensional. We note that the operator $N^{\prime}\in \mathcal{C}l (U\oplus U^{\prime},q|_{U\oplus U^{\prime}})$ and under the isomorphism $\mathcal{C}l (U\oplus U^{\prime},q|_{U\oplus U^{\prime}})\simeq Mat_4(\Q)$, the operator $N^{\prime}$ corresponds to a matrix with only the upper right entry non-zero acting on $\mathcal{C}l (U\oplus U^{\prime},q|_{U\oplus U^{\prime}})$ by left multiplication. This helps us write down a bases for the image which is $12$ dimensional containing the kernel of $N^{\prime}$ which is $4$ dimensional. The kernel and the image consists of all the matrices in $M_4(\Q)$ that look like 
%$$\ker N^\prime =\begin{pmatrix}
%0&*&*&*\\
 %0&*&*&*\\
 %0&*&*&*\\

  %  0&*&*&*\\
    
  

   
%\end{pmatrix}
% \text{ and  }
%im N^\prime =\begin{pmatrix}
%0&0&0&*\\
 %0&0&0&*\\
 %0&0&0&*\\

  %  0&0&0&*\\
   % \end{pmatrix}$$
    %Thus, $W_1 H/W_0 H$ is isomorphic to $(M_2(\Q)\otimes V^{\prime\prime})\otimes \C l(V^{\prime},q|_{U\oplus U^{\prime}})$ where $V^{\prime\prime}$ is $2$ dimensional over $\Q.$ We know that $M_2(\Q)$ is isomorphic to the the clifford algebra generated by orthogonal vectors $e_1, e_2$ with $q(e_1,e_1) = q(e_2,e_2) = 1$ and $q(e_1,e_2)=0$. Hence $J =e_1e_2$ induces a weight one hodge structure on $M_2(\Q)$. Further note that $M_2(\Q)$ splits as a direct sum of weight one Hodge structures $V_1 = \langle{e_1,e_2\rangle}$ and $V_2 = \langle{1,e_1e_2}\rangle$. Moreover, the elliptic curves corresponding to these Hodge structures are isogenous since the $\Q$-lattices are homothetic, that is, $e_1\cdot V_1 =V_2$.  As $W_1 H/W_0 H = M_2(\Q)\otimes V^{\prime\prime}\otimes \C l(V^{\prime})$ is a weight one hodge structure, we see that it corresponds up to isogeny, to a product of $d/2$ copies of an  elliptic curve $E$ over $\mathbb{C}.$
%\end{proof}

%\textcolor{purple}{How do we go from char $0$ to the set up in char $p$? See Ananth's paper on picard ranks over function fields I guess, you get a universal abelian scheme over the GSpin Shimura variety over $\F_p$ so it makes sense to take a $K$-point of of $M$ which gives us $KS(X)$ over $K$}
% \begin{lem}
%Suppose $X$ is a generically ordinary $K3$ surface over $K$. Then the associated Kuga Satake abelian variety $KS(X)$ is ordinary. Furthermore the Raynaud extension of $KS(X)$ satisfies proposition \ref{raynaudk3} with $A_{KS}$ a product of $d/2$ copies if an ordinary elliptic curve.
% \end{lem}

% \begin{proof}
%Note that $KS(X)$ has bad reduction and therefore, has to be generically ordinary.
% \end{proof}
 \section{case of abelian surfaces with real multiplication}
In this section, we generalise the proof by formal groups to the case of certain abelian surfaces with real multiplication. Throughout this section we let $A$ be a generically ordinary abelian surface over $K$ with RM by $\Q(\sqrt{p})$ such that its special fibre is super-singular. Let $\alpha$ denote the morphism such that $\alpha^2 = [p].$ Let $\mathscr{G}$ denote its $p$-divisible group and let $\widehat{\mathscr{G}}$ be its formal group over $K$. We choose a coordinates   $x_1$  and $x_2$ such that $x_2 = \alpha\cdot x_1.$ Further we write the multiplication by $p$ map in these coordinates as 
$$[p]\cdot x_1 = p_1(x_1,x_2) \text{ and  } [p]\cdot x_2 = p_2(x_1, x_2)$$
This gives us that 
$$\alpha\cdot x_1 = x_2 \text{ and } \alpha\cdot x_2 = [p] \cdot x_2 $$
where 
$$p_1(x_1, x_2)= A_{1,0}(t)x^p +A_{0,1}(t)x_2^{p}+A_{1,1}$$



$$p_2(x_1, x_2)$$
We consider the $\alpha$-torsion which is given by $x_2 = 0$ and $p_2(x_1,0) = 0.$




